Super-resolution on network telemetry time series

Fine-grained monitoring is crucial for multiple data-driven tasks such as debugging, provisioning, and securing networks. Yet, practical constraints in collecting, extracting, and storing data often force operators to use coarse-grained sampled monitoring, degrading the performance of the various tasks. In this work, we explore the feasibility of leveraging the correlations among coarse-grained time series to impute their fine-grained counterparts in software. We present Zoom2Net, a transformer-based model for network imputation that incorporates domain knowledge through operational and measurement constraints, ensuring that the imputed network telemetry time series are not only realistic but also align with existing measurements and are plausible. This approach enhances the capabilities of current monitoring infrastructures, allowing operators to gain more insights into system behaviors without the need for hardware upgrades. We evaluate Zoom2Net on four diverse datasets (e.g. cloud telemetry and Internet data transfer) and use cases (such as bursts analysis and traffic classification). We demonstrate that Zoom2Net consistently achieves high imputation accuracy with a zoom-in factor of up to 100 and performs better on downstream tasks compared to baselines by an average of 38%.

==> 2_background.tex <==
\section{Background}
\myitem{Transformer}


\myitem{Physics Informed Neural Networks}


==> related_work.tex <==
\section{Related Work}

\myitem{Signal processing:}
In the realm of signal processing and information theory, there are abundant techniques and theorems for signal compression and reconstruction. 
Nyquist–Shannon sampling theorem states a sampling rate above which the sampled signal can be fully reconstructed. 
However, we find the coarse-grained data we focus on is sampled way below Nyquist rate, making it impossible to be recovered using the theorem.
Compressive sensing is a technique that can recover signals sampled at a rate below Nyquist rate and has been used in sketch algorithm~\cite{huang2021nze} and traffic matrices~\cite{zhang2009spatio}. 
However, compressive sensing requires sparsity and incoherence in the signal, which does not always hold for general network measurement data. Plus, it does not incorporate spatial and temporal correlations which are important factors in reconstructing network signals.  
Another sub-Nyquist sampling method is lossy compression which uses a specific sampling method (\ie discrete cosine transform) that provides a lower bound for the minimal reconstruction error.
However, this sampling is not feasible in today's measurement tools. Consequently, signal processing tools cannot be easily generalized to network measurement data.




Works on synthetic trace generation~\cite{yin2022netshare, lin2020dp} aim to generate packet and flow header traces for networking tasks. The generated data is fine-grained and can be used as \sys's training data.
Network performance estimation works~\cite{zhang2021mimicnet, yang2022deepqueuenet} target to simulate scalable and generalized packet-level simulation and obtain fine-grained performance results. 





